First-order Policy Optimization for Robust Markov Decision Process

We consider the problem of solving robust Markov decision process (MDP), which involves a set of discounted, finite state, finite action space MDPs with uncertain transition kernels. The goal of planning is to find a robust policy that optimizes the worst-case values against the transition uncertainties, and thus encompasses the standard MDP planning as a special case. For $(\mathbf{s},\mathbf{a})$-rectangular uncertainty sets, we establish several structural observations on the robust objective, which facilitates the development of a policy-based first-order method, namely the robust policy mirror descent (RPMD). An $\mathcal{O}(\log(1/\epsilon))$ iteration complexity for finding an $\epsilon$-optimal policy is established with linearly increasing stepsizes. We further develop a stochastic variant of the robust policy mirror descent method, named SRPMD, when the first-order information is only available through online interactions with the nominal environment. We show that the optimality gap converges linearly up to the noise level, and consequently establish an $\tilde{\mathcal{O}}(1/\epsilon^2)$ sample complexity by developing a temporal difference learning method for policy evaluation. Both iteration and sample complexities are also discussed for RPMD with a constant stepsize. To the best of our knowledge, all the aforementioned results appear to be new for policy-based first-order methods applied to the robust MDP problem.

==> robust_pi.tex <==
%!TEX root = ./robust_rl.tex


\section{Robust Policy Iteration}
Consider the robust policy iteration with the following update:
\begin{align}\label{rpi_update}
\pi_{k+1} (\cdot| s) =
	\argmin_{p(\cdot|s) \in \Delta_{\abs{\cA}}}   \inner{Q_r^{\pi_k}(s, \cdot)}{ p(\cdot| s ) }  ,  ~ \forall s \in \cS.
\end{align}
By the optimality condition of the update \eqref{rpi_update}, 
\begin{align}\label{eq_decomp_policy_iter}
\underbrace{\inner{Q^{\pi_k}_r}{\pi_{k+1}}_s
-  \inner{Q^{\pi_k}_r}{\pi_{k}}_s}_{(A)}
+ \underbrace{\inner{Q^{\pi_k}_r}{\pi_{k}}_s
- \inner{Q^{\pi_k}_r}{\pi^*}_s}_{(B)} \leq 0.
\end{align}
In addition, we let $u_k = u_{\pi_k}$ denote the worst-case uncertainty of policy $\pi_k$.

To bound term $(A)$, we observe that 
\begin{align}
V^{\pi_{k+1}}_r(s) - V^{\pi_k}_r(s)
& \leq \frac{1}{1-\gamma} \EE_{s' \sim d^{\pi_{k+1}, u_{k+1}}_{s}} \nonumber
\inner{Q^{\pi_k}_r}{\pi_{k+1} - \pi_k}_{s'} \nonumber\\
& \leq \frac{d^{\pi_{k+1}, u_{k+1}}_{s}(s)}{1-\gamma}  \inner{Q^{\pi_k}_r(s, \cdot)}{\pi_{k+1}(\cdot|s) - \pi_k(\cdot|s)} \nonumber\\
& \leq \inner{Q^{\pi_k}_r(s, \cdot)}{\pi_{k+1}(\cdot|s) - \pi_k(\cdot|s)} \leq 0, \label{rpi_monotone}
\end{align}
where the first inequality is due to Lemma \ref{lemma_perf_diff}; the second inequality is due to the optimality condition of update \eqref{rpi_update}, which further implies $\inner{Q^{\pi_k}_r(s', \cdot)}{\pi_{k+1}(\cdot|s') - \pi_k(\cdot|s')}$ for all $s' \in \cS$;
the third inequality is due to the observation $d^{\pi_{k+1}, u_{k+1}}_{s}(s) \geq (1-\gamma)$ for all $s\in \cS$.

To bound terms $(B)$, we make use of Lemma \ref{lemma_q_signal}.
Specifically,  we obtain from \eqref{ineq_q_signal} that
\begin{align}\label{rpi_vi}
\EE_{s' \sim d_s^{\pi^*, u_{k}}} \sbr{
 \inner{Q^{\pi_k}_r }{\pi_k - \pi^*}_{s'} 
 } 
 \geq 
  (1-\gamma) \rbr{V_r^{\pi}(s) - V^{\pi^*}_r(s)  } \geq 0.
\end{align}

Hence by aggregating \eqref{eq_decomp_policy_iter} across different states with weights set as $ d_s^{\pi^*, u_k}$, and making use of  \eqref{rpi_monotone} and \eqref{rpi_vi}, 
we obtain 
\begin{align*}
\EE_{s' \sim d_s^{\pi^*, u_k}} \rbr{ V_r^{\pi_{k+1}}(s') - V_r^{\pi_k}(s') }
+ (1-\gamma) \rbr{ V^{\pi_{k}}(s) - V^{\pi^*}(s) } 
\leq 0.
\end{align*}
Further taking expectation w.r.t. $s \sim \rho$ in the prior relation, where $\mathrm{supp}(\rho) = \cS$, 
we have 
\begin{align*}
\EE_{s \sim d_{\rho}^{\pi^*, u_k}} \rbr{ V^{\pi_{k+1}}_r(s) - V^{\pi_k}_r(s) }
+ (1-\gamma) \rbr{ f_\rho(\pi_k) - f_\rho (\pi^*) } \leq 0.
\end{align*}
Combined with the fact that $V^{\pi_{k+1}}_r (s) \leq V^{\pi_k}_r(s)$ given \eqref{rpi_monotone}, and the definition of $M \coloneqq \sup_{u \in \cU} \norm{d_\rho^{\pi^*, u} / \rho}_\infty < \infty$, we obtain 
\begin{align*}
& M \sbr{ f_\rho(\pi_{k+1}) - f_\rho(\pi_k) } 
+ (1-\gamma) \sbr{ f_\rho(\pi_k) - f_\rho (x^*) } \leq 0,
\end{align*}
which, after simple arrangement, gives 
\begin{align}
f_\rho (\pi_{k+1}) - f_\rho (x^*) \leq 
(1 - \frac{1-\gamma}{M}) (f_\rho (\pi_k) - f_\rho (x^*)) 
 .\label{recursion_rpi}
\end{align}
 By telescoping \eqref{recursion_rpi}, we obtain
$
f_\rho (\pi_k) - f_\rho (x^*) 
\leq (1 - \frac{1-\gamma}{M})^k \rbr{  f_\rho (\pi_0) - f_\rho (x^*)   }.
$



\newpage

